What's Behind the Mask: Estimating Uncertainty in Image-to-Image Problems

Estimating uncertainty in image-to-image networks is an important task, particularly as such networks are being increasingly deployed in the biological and medical imaging realms. In this paper, we introduce a new approach to this problem based on masking. Given an existing image-to-image network, our approach computes a mask such that the distance between the masked reconstructed image and the masked true image is guaranteed to be less than a specified threshold, with high probability. The mask thus identifies the more certain regions of the reconstructed image. Our approach is agnostic to the underlying image-to-image network, and only requires triples of the input (degraded), reconstructed and true images for training. Furthermore, our method is agnostic to the distance metric used. As a result, one can use $L_p$-style distances or perceptual distances like LPIPS, which contrasts with interval-based approaches to uncertainty. Our theoretical guarantees derive from a conformal calibration procedure. We evaluate our mask-based approach to uncertainty on image colorization, image completion, and super-resolution tasks, demonstrating high quality performance on each.

==> floats/alg_calibration.tex <==
\begin{algorithm}[H]
\caption{\label{alg:calibration}Finding $\lambda_i$}
\centering
\begin{minted}{python}
def scale(lambda_, mask, eps=1e-6):
    return (mask * lambda_ / (eps + mask * (1 - mask))).clip(0, 1)

def find_lambda(mask, y, y_hat, eps=1e-4):
    l, h, lambda_ = eps, 1 / eps, 0

    while h - l > eps:
        lambda_ = (h + l) / 2

        loss = loss_fn(
            y * scale(a, mask),
            y_hat * scale(a, mask))

        if loss > alpha:
            h = lambda_
        else:
            l = lambda_

    return lambda_
\end{minted}
\end{algorithm}

==> floats/fig_cats.tex <==
\begin{figure}
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=.25\textwidth]{imgs/cat.png}
        & \includegraphics[width=.25\textwidth]{imgs/cat-d.png}
    \end{tabular}

    \caption{\label{fig:cats}These two images are identical at 90\% of the pixels, the rest of the 10\% pixels, however, create a perceptual distortion that is quite noticeable a LPIPS score of $0.2758$ confirms this.}
\end{figure}

==> floats/fig_extreme_ci.tex <==
\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[width=4.5cm, ybar, title=a] 
        \addplot+ coordinates {(0, 0.0499) (0.5, 0.9502) (1, 0.0499)};
        \addplot+ coordinates {(0, 0.0501) (0.5, 0.9498) (1, 0.0501)};
        \end{axis}
        
        \begin{axis}[xshift=4.5cm, width=4.5cm, ybar, title=b] 
        \addplot+ coordinates {(0.4, 0.5) (0.6, 0.5)};
        \end{axis}

        \begin{axis}[xshift=9cm, width=4.5cm, ybar, title=c] 
        \addplot+ coordinates {(0, 0.0501) (0.5, 0.9498) (1, 0.0501)};
        \end{axis}
    \end{tikzpicture}
    
    \caption{
    \label{fig:extreme-ci}
        Consider the two distributions in diagram a. The first one has $p(0.5) = 0.9502$ while the scond has $p(0.5) = 0.9498$ yet the 90\% confidence interval for the first distribution is $[0, 1]$, the largest possible, while the 90\% confidence interval for the second distribution is $[\frac{1}{2}, \frac{1}{2}]$, the smallest possible.
        Now consider the two distributions on diagram b and c, their 90\% confidence interval and the expected absolute error are $[0.4, 0.6]$, $0.1$ and $[0, 1]$, $0.0501$ respectively, so the distribution on diagram b is associated with larger distortion but smaller confidence interval.
        }
\end{figure}

==> floats/fig_hist.tex <==
\begin{figure}[b]
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=.5\textwidth]{imgs/size_hist_completion_gan_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_hist_completion_gan_lpips.pdf} \\
        \includegraphics[width=.5\textwidth]{imgs/size_hist_completion_regressor_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_hist_completion_regressor_lpips.pdf}
    \end{tabular}

    \caption{Image Completion - Histograms}
\end{figure}


\begin{figure}[b]
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=.5\textwidth]{imgs/size_hist_sr_gan_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_hist_sr_gan_ssim.pdf} \\
        \includegraphics[width=.5\textwidth]{imgs/size_hist_sr_regressor_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_hist_sr_regressor_ssim.pdf}
    \end{tabular}

    \caption{Super Resolution- Histograms}
\end{figure}

\begin{figure}[b]
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=.5\textwidth]{imgs/size_hist_color_gan_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_hist_color_gan_l2.pdf} \\
        \includegraphics[width=.5\textwidth]{imgs/size_hist_color_regressor_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_hist_color_regressor_l2.pdf}
    \end{tabular}

    \caption{Colorization - Histograms}
\end{figure}


\begin{figure}[b]
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=.5\textwidth]{imgs/size_corr_completion_gan_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_corr_completion_gan_lpips.pdf} \\
        \includegraphics[width=.5\textwidth]{imgs/size_corr_completion_regressor_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_corr_completion_regressor_lpips.pdf}
    \end{tabular}

    \caption{Image Completion - Correlation}
\end{figure}


\begin{figure}[b]
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=.5\textwidth]{imgs/size_corr_sr_gan_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_corr_sr_gan_ssim.pdf} \\
        \includegraphics[width=.5\textwidth]{imgs/size_corr_sr_regressor_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_corr_sr_regressor_ssim.pdf}
    \end{tabular}

    \caption{Super Resolution- Correlation}
\end{figure}

\begin{figure}[b]
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=.5\textwidth]{imgs/size_corr_color_gan_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_corr_color_gan_l2.pdf} \\
        \includegraphics[width=.5\textwidth]{imgs/size_corr_color_regressor_l1.pdf}
        & \includegraphics[width=.5\textwidth]{imgs/size_corr_color_regressor_l2.pdf}
    \end{tabular}

    \caption{Colorization - Correlation}
\end{figure}

==> floats/fig_methods.tex <==
\begin{figure}
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=.48\textwidth]{imgs/sr_regressor_l1.pdf}
        \includegraphics[width=.48\textwidth]{imgs/sr_gan_ssim.pdf}
        \\
        \includegraphics[width=.48\textwidth]{imgs/completion_regressor_l1.pdf}
        \includegraphics[width=.48\textwidth]{imgs/completion_regressor_lpips.pdf}
    \end{tabular}
    \begin{tabular}{c c c}
        \includegraphics[width=.31\textwidth]{imgs/loss_sr_gan_ssim.pdf}
        \includegraphics[width=.31\textwidth]{imgs/loss_completion_regressor_l1.pdf}
        \includegraphics[width=.31\textwidth]{imgs/loss_completion_regressor_lpips.pdf}
    \end{tabular}

    \caption{\label{fig:methods}
        The four top charts depict the calibrated mask size with respect to the distortion of the random sample.
        The three bottom charts show the distribution of the masked distortion.}
\end{figure}

==> floats/fig_mri.tex <==
\begin{figure}
\centering
\scalebox{.3}{\includegraphics{imgs/mri.png}}
\caption{
An example of conformal prediction in the context of image to image translation.
The model predicts an interval of values per pixel and by taking the mean of the interval and its size we can produce images B. and C. respectively. 
\label{fig:mri}}
\end{figure}

==> floats/fig_ssim.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{imgs/ssim.png}
    \caption{Caption}
    \label{fig:ssim}
\end{figure}

==> floats/tab_completion.tex <==
\begin{table}
    \centering
    \begin{tabular}{c c||c|c|c||c|c||c|c}
        & & \multicolumn{3}{c||}{$\mathbf{\| M \| \quad (\downarrow)}$} & \multicolumn{2}{c||}{$\mathbf{C(M, D) \quad (\uparrow)}$} & \multicolumn{2}{c}{$\mathbf{C(M, M_{opt}) \quad (\uparrow)}$} \\
        \cline{3-5}\cline{6-7}\cline{8-9}
        \cline{3-5}\cline{6-7}\cline{8-9}
        Network & Distance & Opt & Ours & Quantile & Ours & Quantile & Ours & Quantile \\
        \hline\hline
        Regression & L1 & $0.09$ & \best{0.10} & $0.15$ & \best{0.89} & $0.78$ & \best{0.89} & $0.76$ \\
        \hline
        Regression & LPIPS & $0.01$ & \best{0.01} & $0.20$ & \best{0.54} & $0.51$ & \best{0.89} & $0.77$ \\
        \hline
        GAN & L1        & $0.09$ & \best{0.09} & $0.14$ & \best{0.95} & $0.85$ & \best{0.94} & $0.80$ \\
        \hline
        GAN & LPIPS        & $0.01$ & \best{0.01} & $0.08$ & \best{0.31} & $0.24$ & \best{0.50} & $0.23$
    \end{tabular}
    \caption{Image Completion Results.  $\|M\|$ indicates average mask size; $C(M, D)$ the correlation between predicted mask size and the amount of distortion; and $C(M, M_{opt})$ the correlation between the size of the calibrated mask and the size of the optimal mask.  Arrows indicate which direction is better.  Best results shown in \textcolor{blue}{\textbf{blue}}.}
    \label{tab:completion-results}
\end{table}


        % \\\cmidrule(lr){3-6}\multirow{4}*{Image Completion} 
        %         & \multirow{2}*{Regression}    
        %                 &   L1     & $0.09$ & $0.89/0.10/0.89$ & $0.78/0.15/0.76$
        %             \\  &&  LPIPS  & $0.01$ & $0.54/0.01/0.89$ & $0.51/0.20/0.77$
            
        %     \\\cmidrule(lr){3-6} & \multirow{2}*{GAN}    
        %                 &   L1     & $0.09$ & $0.95/0.09/0.94$ & $0.85/0.14/0.80$
        %             \\  &&  LPIPS  & $0.01$ & $0.31/0.01/0.50$ & $0.24/0.08/0.23$


==> floats/tab_l1.tex <==
\begin{table}
\centering
\begin{tabular}{lcccccc}

\toprule
& \multicolumn{2}{c}{Colorization} 
& \multicolumn{2}{c}{Image Completion}  
& \multicolumn{2}{c}{Super Resolution} 
\\      
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
& Regressor & GAN                
& Regressor & GAN                       
& Regressor & GAN
\\\midrule
L1 & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$
\\
LPIPS & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$
\\
DISTS & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$

\\\bottomrule
\end{tabular}

\caption{
\label{tab:l1}
\todo{}}
\end{table}

==> floats/tab_l1corr.tex <==
\begin{table}
\centering
\begin{tabular}{lcccc}

\toprule
& \multicolumn{2}{c}{LPIPS} 
& \multicolumn{2}{c}{DISTS}  
\\      
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
& Regressor & GAN                
& Regressor & GAN                       
\\\midrule
L1 & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$

\\\bottomrule
\end{tabular}

\caption{\label{tab:l1corr}
\todo{Caption}}
\end{table}

==> floats/tab_mask_eval1.tex <==
\begin{table}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{rcccc}
        \toprule
        &&& Predicted & Optimal 
        \\ \midrule
        \multirow{2}*{Colorization} & GAN & L1 & $0.66$ & $0.65$  
        \\ & GAN & L2  & $0.54$ & $0.52$ 
        \\ \midrule
        \multirow{2}*{Image Completion} & \multirow{2}*{GAN} & L1  & $99\pm 99$ 
        \\ && DISTS  & $99\pm 99$ 
        \\ \midrule
        \multirow{2}*{Super Resolution} & Regression & L1  & $99\pm 99$ 
        \\ & GAN & L1  & $99\pm 99$ 
        \\ \bottomrule
    \end{tabular}
    \caption{\label{tab:mask-eval1}Caption}
\end{table}

==> floats/tab_mask_size.tex <==
\begin{table}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{rccccc}
        \toprule
        &&& Our   & UNI & GRAD
        \\ \midrule
        \multirow{2}*{Colorization} & Regression & L1 & $99\pm 99$  & $99\pm 99$ & $99\pm 99$
        \\ & GAN & LPIPS  & $99\pm 99$ & $99\pm 99$ & $99\pm 99$
        \\ \midrule
        \multirow{2}*{Image Completion} & \multirow{2}*{GAN} & L1  & $99\pm 99$ & $99\pm 99$ & $99\pm 99$
        \\ && DISTS  & $99\pm 99$ & $99\pm 99$ & $99\pm 99$
        \\ \midrule
        \multirow{2}*{Super Resolution} & Regression & L1  & $99\pm 99$ & $99\pm 99$ & $99\pm 99$
        \\ & GAN & L1  & $99\pm 99$ & $99\pm 99$ & $99\pm 99$
        \\ \bottomrule
    \end{tabular}
    \caption{\label{tab:mask-size}Caption}
\end{table}

==> floats/tab_methods.tex <==
\begin{table}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{rccccc}
        \toprule
        &&& Opt & Ours & Quantile
        \\\cmidrule(lr){3-6}\multirow{4}*{Colorization} 
            & \multirow{2}*{Regression}    
                        &   L1     & $0.55$ & $0.44/0.71/0.40$ & $0.46/0.72/0.34$
                    \\  &&  L2     & $0.47$ & $0.45/0.66/0.37$ & $0.47/0.70/0.24$

            \\\cmidrule(lr){3-6} & \multirow{2}*{GAN}    
                        &   L1     & $0.55$ & $0.45/0.71/0.41$ & $0.39/0.72/0.34$
                    \\  &&  L2     & $0.47$ & $0.45/0.65/0.39$ & $0.39/0.70/0.25$

        \\\cmidrule(lr){3-6}\multirow{4}*{Image Completion} 
                & \multirow{2}*{Regression}    
                        &   L1     & $0.09$ & $0.89/0.10/0.89$ & $0.78/0.15/0.76$
                    \\  &&  LPIPS  & $0.01$ & $0.54/0.01/0.89$ & $0.51/0.20/0.77$
            
            \\\cmidrule(lr){3-6} & \multirow{2}*{GAN}    
                        &   L1     & $0.09$ & $0.95/0.09/0.94$ & $0.85/0.14/0.80$
                    \\  &&  LPIPS  & $0.01$ & $0.31/0.01/0.50$ & $0.24/0.08/0.23$

        \\\cmidrule(lr){3-6}\multirow{4}*{Super Resolution} 
                & \multirow{2}*{Regression}    
                        &   L1      & $0.24$ & $0.99/0.26/0.95$ & $0.54/0.28/0.88$
                    \\  &&  SSIM    & $0.03$ & $0.66/0.03/0.82$ & $0.64/0.13/0.57$
            
            \\\cmidrule(lr){3-6} & \multirow{2}*{GAN}    
                        &   L1      & $0.26$ & $0.94/0.30/0.80$ & $0.63/0.40/0.72$
                    \\  &&  SSIM    & $0.03$ & $0.79/0.03/0.83$ & $0.63/0.13/0.63$
        
        \\ \bottomrule
    \end{tabular}
    \caption{\label{tab:methods}
        \todo{Gilad: SR}
        For Opt we report the average mask size, for Our and Quantile the reported numbers from left to right are the correlation between predicted mask size and the amount of distortion, the average mask size and the correlation between the size of the calibrated mask and the size of the Opt mask.}
        
\end{table}

==> floats/tab_model_eval.tex <==
\begin{table}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{rccc}
        \toprule
        && MAE   & FID 
        \\ \midrule
        \multirow{2}*{Colorization} & Regression & $0.039\pm0.023$ & 7.91
        \\ & GAN & $0.039\pm0.023$ & 7.14
        \\ \midrule
        \multirow{2}*{Image Completion} & Regression & $0.023\pm0.009$  & $21.89$
        \\ & GAN & $0.029\pm0.012$ & $22.66$
        \\ \midrule
        \multirow{2}*{Super Resolution} & Regression & $0.043\pm0.009$  & NA
        \\ & GAN & $0.043\pm0.009$ & NA
        \\ \bottomrule
    \end{tabular}
    \caption{\label{tab:model-eval}Note that $\pm$ here denotes the standard deviation, also, for the colorization task, metrics were computed in RGB color space.}
\end{table}

==> floats/tab_sr.tex <==
\begin{table}
    \centering
    \begin{tabular}{c c||c|c|c||c|c||c|c}
        & & \multicolumn{3}{c||}{$\mathbf{\| M \| \quad (\downarrow)}$} & \multicolumn{2}{c||}{$\mathbf{C(M, D) \quad (\uparrow)}$} & \multicolumn{2}{c}{$\mathbf{C(M, M_{opt}) \quad (\uparrow)}$} \\
        \cline{3-5}\cline{6-7}\cline{8-9}
        \cline{3-5}\cline{6-7}\cline{8-9}
        Network & Distance & Opt & Ours & Quantile & Ours & Quantile & Ours & Quantile \\
        \hline\hline
        Regression & L1 & $0.24$ & \best{0.26} & $0.28$ & \best{0.99} & $0.54$ & \best{0.95} & $0.88$ \\
        \hline
        Regression & SSIM & $0.03$ & \best{0.03} & $0.13$ & \best{0.66} & $0.64$ & \best{0.82} & $0.57$ \\
        \hline
        GAN & L1        & $0.26$ & \best{0.30} & $0.40$ & \best{0.94} & $0.63$ & \best{0.80} & $0.72$ \\
        \hline
        GAN & SSIM        & $0.03$ & \best{0.03} & $0.13$ & \best{0.79} & $0.63$ & \best{0.83} & $0.63$
    \end{tabular}
    \caption{Super Resolution Results.  $\|M\|$ indicates average mask size; $C(M, D)$ the correlation between predicted mask size and the amount of distortion; and $C(M, M_{opt})$ the correlation between the size of the calibrated mask and the size of the optimal mask.  Arrows indicate which direction is better.  Best results shown in \textcolor{blue}{\textbf{blue}}.}
    \label{tab:sr-results}
\end{table}

        % \\\cmidrule(lr){3-6}\multirow{4}*{Super Resolution} 
        %         & \multirow{2}*{Regression}    
        %                 &   L1      & $0.24$ & $0.99/0.26/0.95$ & $0.54/0.28/0.88$
        %             \\  &&  SSIM    & $0.03$ & $0.66/0.03/0.82$ & $0.64/0.13/0.57$
            
        %     \\\cmidrule(lr){3-6} & \multirow{2}*{GAN}    
        %                 &   L1      & $0.26$ & $0.94/0.30/0.80$ & $0.63/0.40/0.72$
        %             \\  &&  SSIM    & $0.03$ & $0.79/0.03/0.83$ & $0.63/0.13/0.63$


==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> old/abstract_1.tex <==
Uncertainty estimation in image reconstruction tasks is of extreme importance especially in domains such as biological and medical imaging. 
We propose a unified approach that learns directly the uncertain regions in the predicted image.
Our approach is agnostic to the underlying model and only requires triplets of the degraded, predicted and reference images.
It can be used with many common distortion criteria and by conducting a simple calibration procedure, our method yield strong statistical guarantees. 
We evaluate our procedure on three image reconstruction tasks: image colorization, image completion and image super-resolution.
Our uncertainty estimations are highly correlated with the true distortion, we are able to produce prediction sets that are much smaller than the one obtained by a straight forward approach and we show that our solution has high adaptivity to the input.
We make our data-sets public to promote further research on this topic.

==> old/experiments_1.tex <==
% \textbf{List of TODO's}

% \begin{itemize}
    %\item \todo{\sout{Compare to Yaniv}}
    %\item \todo{\sout{Chart - show that we get the guarantee}}
    %\item \todo{\sout{Chart mask size vs distortion}}
    % \item \todo{Visualize masks on different distortions e.g. colorization l1 vs lpips}
    % \item \todo{Visualize images with large distortion vs images with low distortions}
    % \item \todo{Gilad: figure $x, y, y_hat, |y - y_hat|, m$ for each one of the tasks}
    % \item \todo{Gilad: generate optimal mask size vs our, quantile mask size graphs for 12 combinations}
    % \item \todo{Gilad: generate histogram of the mask size for each of the 12 combinations}
% \end{itemize}

\subsection{Datasets and Tasks}

\parbasic{Datasets} Two data-sets are used in our experiments:

\begin{addmargin}[1em]{0em}% 1em left, 0em right

\category{Places365} \citep{places365}: A large collection of 256x256 images from 365 scene categories. We use 1,803,460 images for training and 36,500 images for validation/test.

\category{Rat Astrocyte Cells} \citep{rat}: A dataset of 1,200 uncompressed images of scanned rat cells of resolution 990$\times$708.  We crop the images into 256$\times$256 tiles, and randomly split them into train and validation/test sets of sizes 373,744 and 11,621 respectively.
The tiles are partially overlapped as we use stride of 32 pixels when cropping the images.

\end{addmargin}

\parbasic{Tasks} We consider the following image-to-image tasks:

\begin{addmargin}[1em]{0em}% 1em left, 0em right

\category{Completion}:
Using grayscale version of Places365, we remove a middle vertical and horizontal stripe of 32 pixel width, and aim to reconstruct the missing part.

\category{Super Resolution}:
Using the Rat Astrocyte Cells dataset, we downscale the tiles to 64$\times$64 images, and aim to reconstruct the original tile.

\category{Colorization}:
We convert the Places365 images to grayscale and aim to recover their colors.

\end{addmargin}

Figure~\ref{fig:tasks} shows a sample input and output for each of the above tasks.
\input{floats/fig_tasks}


\subsection{Experimental Details and Settings}

\parbasic{Image-to-Image Models} We start by training models for the above three tasks.  Note that these models are not intended to be state of the art, but rather used to demonstrate the uncertainty estimation technique proposed in this work. We use the same model architecture for all tasks: an 8 layer U-Net.
For each task we train two versions of the network: (i) A simple regressor; and (ii) A conditional GAN, where the generator plays the role of the reconstruction network. 
%As in \citet{pix2pix} the generator observes the input but it does not have an access to a random noise.
For the GAN, the discriminator is implemented as a 4 layer CNN. We use the L1 loss as the objective for the regressor, and augment it with an adversarial loss in the conditional GAN ($\lambda = 20$), as in \citet{pix2pix}.
%, that is:
%\begin{equation}
%     \arg \min_G \max_D \mathcal{L}_{\text{cGAN}}(G, D) + \lambda\mathcal{L}_\text{L1}(G)
% \end{equation}
% where
% \begin{equation}
%     \mathcal{L}_{\text{cGAN}}(G, D) = \mathbb{E}_{x,y}[\log D(x, y)] + \mathbb{E}[\log(1 - d(x, G(x, y)))].
% \end{equation}
% and we set $\lambda = 20$.
All models are trained for two epochs using the Adam optimizer with a learning rate equal to $1\text{e-}5$ and a batch size equal to $50$. % In Table~\ref{tab:model-eval} we report the performance of these models in terms of mean absolute error (MAE) as well as the FID score \citep{fid} where applicable.

% \input{floats/tab_model_eval}

\parbasic{Mask Model} For our masking model we also use an 8 layer U-Net architecture.  This choice was made for simplicity and compatibility with previous work.  The masking model is trained using the predictions of the image-to-image model with the loss function described in Section \ref{sec:method} with $\mu=2$, learning rate of $1\text{e-}5$ and a batch size of 25.

\parbasic{Experiments} We consider the L1, L2, SSIM and LPIPS distances.
We set aside $1,000$ samples from each validation set for calibration and use the remaining samples for evaluation.  
We demonstrate the flexibility of our approach by conducting experiments on a variety of $12$ settings: (i) Image Completion: \{Regressor, GAN\} $\times$ \{L1, LPIPS\}; (ii) Super Resolution: \{Regressor, GAN\} $\times$ \{L1, SSIM\}; and (iii) Colorization: \{Regressor, GAN\} $\times$ \{L1, L2\}.

\parbasic{Thresholds} Recall that given a predicted image, our goal is to find a mask that, when applied to both the prediction and the (unknown) reference image, reduces the distortion between them to a predefined threshold with high probability $\beta$.
Here we fix $\beta = 0.9$ and choose the threshold to be the $0.1$-quantile of each measure computed on a random sample from the validation set, i.e. roughly $10\%$ of the predictions are already considered sufficiently good and do not require masking at all.

\subsection{Competitor Techniques}

\parbasic{Quantile -- Interval-Based Technique} We compare our method to the quantile regression option presented in \citep{angelopoulos2022image}. As described in Section \ref{sec:prior}, their uncertainty is formulated by pixel-wise confidence intervals, calibrated so as to guarantee that with high probability the true value of the image is indeed within the specified range. 
While their predicted confidence intervals are markedly different from the expected distortion we consider, we can use these intervals as a heuristic mask. 
% \todo{Explain how the heuristic mask is computed based on the intervals.}
For completeness, we also report the performance of the quantile regression even when it is less suitable, i.e. when the underlying model is a GAN and when the distortion loss is different from L1.
We note again that for the sake of a fair comparison, our implementation of the masking model uses exactly the same architecture as the quantile regressor.

\parbasic{Opt -- Oracle} We also compare our method with an oracle, denoted Opt, which computes an optimal mask using the following optimization procedure that has access to the reference image $y$:
\begin{equation}
    \ell(m) =\min_{m} ||m-\vv{1}||_2^2 + \mu d_m(y, \hat{y}).
\end{equation}
This minimization is obtained via gradient descent, using the Adam optimizer with a step-size $0.01$, iterating until the destination distortion value is attained. 
Clearly, this approach does not require calibration, as the above procedure ensures that all the masked samples are below the target distortion threshold.

\subsection{Results \& Discussion}

We now turn to bring series of results that demonstrate our proposed uncertainty masking approach, and its comparison with Opt and Quantile.\footnote{Due to space limitation, we bring all the experimental results in Appendix B, while presenting a selected portion of them here.} Figure \ref{fig:visual} starts by providing a representative visual illustration of our proposed mask for several test cases. As can be seen, the mask aligns well with the true prediction error, while still identifying sub-regions of high certainty. 

% \todo{LPIPS vs. L1?}

In Figure \ref{fig:ResultsSummary} we explore the performance of the three compared methods with respect to the probabilistic guarantee, the size of the masks obtained and the correlation between mask sizes -- Quantile and Ours versus Opt. As can be seen from the top row, all three methods meet the distortion threshold with less than $10\%$ exceptions, as required. Naturally, Opt does not have outliers since each mask is optimally calibrated by its computation. The spread of loss-values tends to be higher with Quantile, indicating a weaker performance. The colorization results, here and below, seem to be more challenging, with a smaller performance margin for our method.

The above probabilistic results are not surprising as they are the outcome of the calibration stage. The main question remaining is the size of the mask created so as to meet this threshold distortion. The middle row in Figure \ref{fig:ResultsSummary} presents histograms of these sizes, showing that our approach tends to a mask that is close to Opt, while Quantile has larger, thus inferior, masked area. Again, our colorization results show smaller if any improvement. 

The bottom row in Figure \ref{fig:ResultsSummary} shows the correlation between mask sizes, and as can be observed, a high such correlation exists between Ours and Opt, while Quantile produces less correlated and much darker masks. 

% \begin{addmargin}[1em]{0em}
% (i) \textit{Correlation between the predicted mask size and the distortion it tries to minimize}.  We are interested in this measure as it is a good indicator that the model learns to distinguish between instances with high uncertainty and instances with low uncertainty.
%The first measure we are interested in is the correlation between the predicted mask size and the distortion it tries to minimize as this is a good indicator that the model learns to distinct between instances with high uncertainty and instances with low uncertainty.

% (ii) \textit{Average size of the calibrated masks}: this is of interest as, under the same guarantees, smaller masks are preferred.
%Next, we measure the average size of the calibrated masks as, under the same guarantees, smaller masks are preferred.

% (iii) \textit{Correlation between the size of the calibrated masks and Opt}: this is of interest as higher correlation indicates better adaptivity, see Section~3.1 in \citet{gentle}.
%Finally, we compute the correlation between the size of the calibrated masks and Opt as higher correlation indicates better adaptivity, see Section~3.1 in \citet{gentle}.

% \end{addmargin}

% \parbasic{Discussion of Results}
% \todo{Miki: please have a look at the following, edit as needed.}
We summarize some quantitative results in Table~\ref{tab:colorization-results}
for the completion, super resolution, and colorization tasks. First and foremost, the results obtained by our method surpass those of Quantile across the board. 
% In Table~\ref{tab:methods} we report the results and, as one can see, in many scenarios our model is highly correlated with Opt and it achieves average mask size that is comparable with Opt.
Our method exhibits smaller mask size $\mathbf{\|M\|}$, aligned well with the mask obtained by Opt. Quantile, as expected, produces bigger masks. In terms of the correlation between the obtained mask-size and the un-masked distortion value $\mathbf{C(M, D)}$, our method shows high such agreement, while Quantile lags behind. This correlation indicates a much-desired adaptivity of the estimated mask to the complexity of image content and thus to the induced uncertainty. 
The correlation $\mathbf{C(M, M_{opt})}$ between Opt's mask size and the one obtained by our method or Quantile show similar behavior, aligned well with behavior we see in the bottom of Figure (\ref{fig:ResultsSummary}). 


%It is less flexible and can not be used for general distortion measures.
% Even when the underlying model is a regressor and the target distortion is L1, the predicted intervals are not translated to masks very well.
% the other direction is also true as the method in~\citep{angelopoulos2022image} to obtained confidence interval by predicting the magnitude of residual did not perform very well.
% In Figure~\ref{fig:methods} we plot the size of the calibrated mask with respect to the distortion of a random sample for the super resolution and image completion tasks.

% This, again, demonstrate the flexibility of our method compared to previous ones.
% In addition we plot the the distribution of the masked distortion and verified that the theoretical guarantees are achieved in practice. 
% In theory, the Opt distribution should be concentrated near the threshold (as in the middle chart) but due to the discrete optimization procedure and the chosen learning rate this is only approximated.

\input{floats/fig_visual}

\input{floats/fig_results}

\input{floats/tab_colorization_comp_sr}
% \input{floats/tab_completion}
% \input{floats/tab_sr}
% \input{floats/tab_methods}

% \input{floats/fig_methods}
% \input{floats/tab_colorization}

==> old/main_1.tex <==
\input{macros}

\begin{document}
\maketitle
\begin{abstract}
Uncertainty estimation in image reconstruction tasks is of extreme importance especially in domains such as biological and medical imaging. 
We propose a unified approach that learns directly the uncertain regions in the predicted image.
Our approach is agnostic to the underlying model and only requires triplets of the degraded, predicted and reference images.
It can be used with many common distortion criteria and by conducting a simple calibration procedure, our method yield strong statistical guarantees. 

We evaluate our procedure on three image reconstruction tasks: image colorization, image completion and image super-resolution.
Our uncertainty estimations are highly correlated with the true distortion, we are able to produce prediction sets that are much smaller than the one obtained by a straight forward approach and we show that our solution has high adaptivity to the input.
We make our data-sets public to promote further research on this topic.
\end{abstract}

\section{Introduction}
Uncertainty estimation in image reconstruction tasks is of extreme importance especially in domains such as biological and medical imaging. 
\todo{elaborate}

Conformal prediction\cite{DBLP:gentel} is a general approach and a set of calibration techniques that are used to transform a point prediction into a confidence set.
By doing so we are able to provide strong statistical guarantees.
This approach has been applied to many regression and classification tasks \todo{citations} but until very recently was not utilized in the context of image to image tasks.
\todo{Finish introduction}

\section{Previous Work}
Angelopoulos et al. experiment with the conformal prediction technique and developed a calibration procedure in the context of image to image regression.
They evaluate several models on several medical image to image tasks. 
Their models, in addition to predicting a value per each pixel, also predict a confidence interval and, after calibration, provide the following guarantee:
\begin{equation}
    P\left(\E\left[\frac{1}{MN}\left|\{(m,n) : Y^\text{test}_{(m,n)} \in \mathcal{T}(X^\text{test})_{(m,n))}\}\right|\right] \geq \alpha \right) \geq \beta
\end{equation}
where $\mathcal{T}_{(m,n)}$ is the predicted confidence interval for the $(m,n)$ pixel and $\alpha$ and $\beta$ are user predefined parameters.
In words this means that with high probability a large fraction of the pixels are guaranteed to be within the predicted confidence intervals.
The predicted confidence intervals can be visualized as a uncertainty heat-map as depicted in Fig~\ref{fig:mri}.
\todo{Finish previous work}

\begin{figure}
\centering
\scalebox{.3}{\includegraphics{imgs/mri.png}}
\caption{
An example of conformal prediction in the context of image to image translation.
The model predicts an interval of values per pixel and by taking the mean of the interval and its size we can produce images B. and C. respectively. 
\label{fig:mri}}
\end{figure}

\section{Notation and Goal}
For simplicity of presentation, and without loss of generality, we consider an image to be a $n$-dimensional vector in $[0,1]^n$.
We use $x, y, \hat{y}$ to denote input, target and predicted images respectively.
We abuse notation and consider any operation between a vector and a scalar as the element wise operation, for example, $2 + [1, 2, 3] = [3, 4, 5]$.
We use the $\odot$ operator to denote element-wise multiplication between vectors, i.e. $[1, 2, 3] \odot [4, 5, 6] = [4, 10, 18]$.

A mask $m \in [0, 1]^n$ is also a $n$-dimensional vector.
We say that $m$ \emph{masks} $y$ if we multiply, element-wise, $y$ with $m$, i.e. $y \odot m$.
The \emph{size} of a mask is equal to $1 - \norm{m}_1$, i.e. the mask $\vv{1}$ has size 0 while the mask $\vv{0}$ has size of 1.


We use $d(\cdot, \cdot)$ to denote a general distortion measure between two images and, when sub-scripted with $m$, $d_m(y, \hat{y})$ is the distortion measure of the masked images, i.e. $d_m(y, \hat{y}) = d(y \odot m, \hat{y} \odot m)$


As mentioned before, previous work addressed the uncertainty by constructing a confidence interval for each individual pixel. 
While providing strong guarantees, a confidence interval has some shortcoming: first, it is sensitive to small changes in the distribution, second, it is loosely, if at all, related to the distortion and finally, there are no guarantees on the image as a whole, see Figures~\ref{fig:extreme-ci},\ref{fig:cats} for detailed examples. 

We mitigate these shortcoming by taking a more direct and holistic approach and define the uncertainty as follow:
\begin{equation}
    U(x) = \E_{y|x, \hat{y}|x}[d(y, \hat{y})]
\end{equation}
Given the above definition our goal is to construct a mask, $m \in [0, 1]^n$, such that with high probability the distortion between the masked images is low, more formally:
\begin{equation}
    \label{eq:goal}
    P(\E_{y|x, \hat{y}|x}[d_m(y, \hat{y})] \leq \alpha) \geq \beta
\end{equation}
where the user is free to choose $d$, $\alpha$ and $\beta$.
A high level overview of our approach is illustrated in Figure~\ref{fig:model}.

\todo{is there a connection between $\E_{y|x, \hat{y}|x}[d(y, \hat{y})]$ and $\nabla d$?}

\todo{prove the existence of an image inside the envelop defined by the mask}

\begin{figure}
    \centering
    \begin{tikzpicture}
        \begin{axis}[width=6cm, ybar, title=a] 
        \addplot+ coordinates {(0, 0.0499) (0.5, 0.9502) (1, 0.0499)};
        \addplot+ coordinates {(0, 0.0501) (0.5, 0.9498) (1, 0.0501)};
        \end{axis}
        
        \begin{axis}[xshift=6cm, width=6cm, ybar, title=b] 
        \addplot+ coordinates {(0.4, 0.5) (0.6, 0.5)};
        \end{axis}

        \begin{axis}[xshift=12cm, width=6cm, ybar, title=c] 
        \addplot+ coordinates {(0, 0.0501) (0.5, 0.9498) (1, 0.0501)};
        \end{axis}
    \end{tikzpicture}
    
    \caption{
    \label{fig:extreme-ci}
        Consider the two distributions in diagram a. The first one has $p(0.5) = 0.9502$ while the scond has $p(0.5) = 0.9498$ yet the 90\% confidence interval for the first distribution is $[0, 1]$, the largest possible, while the 90\% confidence interval for the second distribution is $[\frac{1}{2}, \frac{1}{2}]$, the smallest possible.
        Now consider the two distributions on diagram b and c, their 90\% confidence interval and the expected absolute error are $[0.4, 0.6]$, $0.1$ and $[0, 1]$, $0.0501$ respectively, so the distribution on diagram b is associated with larger distortion but smaller confidence interval.
        }
\end{figure}

\begin{figure}
    \centering
    \begin{tabular}{c c}
        \includegraphics[width=.25\textwidth]{imgs/cat.png}
        & \includegraphics[width=.25\textwidth]{imgs/cat-d.png}
    \end{tabular}

    \caption{\label{fig:cats}These two images are identical at 90\% of the pixels, the rest of the 10\% pixels, however, create a perceptual distortion that is quite noticeable a LPIPS score of $0.2758$ confirms this.}
\end{figure}



\section{\label{sec:method}Method}
As in previous work, to construct the uncertainty mask we first output a heuristic notion of uncertainty (the masking model) and then calibrate to obtain strong statistically guarantees.
In this paper we experiment with a simple calibration procedure in which we scale the output by a fixed scalar $\lambda$.
Tough more sophisticated calibration techniques can be considered, we show that this simple procedure yields good results. 

Recall from Equation~\ref{eq:goal} that our objective is to reduce the distortion between the masked images below a given threshold $\alpha$.
A natural choice, then, is to use the gradient of $d_m$ as a guidance to construct the mask, more formally we define our target mask to be:
\begin{equation}
    m = \mathbb{1} - \pdv{d_m}{m}
\end{equation}
Clearly, during test time $m$ is unknown as we don't know $y$, so we need to learn to predict $m$ and we denote by $\hat{m}$ this prediction.
Our objective function during training is the mean absolute error between $m$ and $\hat{m}$:
\begin{equation}
    \label{eq:loss-mask}
    \mathcal{L}_\text{mask} = \frac{|m - \hat{m}|}{n}
\end{equation}

Our calibration procedure is simple and fast.
Using a calibration set $\mathcal{C} = \{(x_1, y_1, \hat{y}_1),  \dots, (x_m, y_m, \hat{y}_m)\}$ we predict a mask $m_i$ for each $(x_i, \hat{y}_i)$, then we find the maximal\footnote{In practice, we allow a margin of up to $\epsilon = $ from the actual maximal value.} $\lambda_i$, such that 
$d(y_i \cdot \lambda_i \cdot m_i, \hat{y} \cdot \lambda_i \cdot m_i) < \alpha$, we make sure that $\lambda_i \cdot m_i \in [0, 1]^n$ by clamping it.
The procedure that finds the appropriate $\lambda_i$ is formally described in Algorithm~\ref{alg:calibration}.
After calculating all the $\lambda_i$s we take the $1 - \beta$ quantile as our final $\lambda$.


\begin{figure}
\centering
\begin{tikzpicture}[on grid]
\newcommand{\dy}{3} 
\newcommand{\dx}{8} 
\newcommand{\minsize}{4mm} 

\tikzstyle{arrow} = [
solid, 
line width = 9pt, 
{Square[round, line width=1pt, length= 2pt, width=9pt]}-{Triangle[width = 18pt, length = 12pt, round, line width=1pt]}, 
color = black!30, 
shorten >= 3pt, 
shorten <= 3pt]

\tikzstyle{empty} = [line width=0, minimum size=0, inner sep=0]

\tikzstyle{l1} = [circle, minimum size=\minsize, fill=orange!30]
\tikzstyle{l2} = [circle, minimum size=\minsize, fill=teal!50]
\tikzstyle{l3} = [circle, minimum size=\minsize, fill=purple!50]

\node[rounded corners=2mm, minimum size=2cm, path picture={
    \node at (path picture bounding box.center){
        \includegraphics[width=2cm]{imgs/color.jpg}};
}] (gray) at (0,0) {};
\node[above=14mm of gray] {$x$};

\draw[arrow] (gray.east) -> +(1,0) node[empty](arr1){};
% MODEL
\node[empty] (input) at(arr1.east) {};

\node[l2, above right=\dy mm and 2mm of input] (l11) {};
\node[l2, below right=\dy mm and 2mm of input] (l12) {};

\node[l2, above right=\dy mm and \dx mm of l11] (l21) {};
\node[above=5mm of l21]{\footnotesize Colorization Model};
\node[l2, below right=\dy mm and \dx mm of l11] (l22) {};
\node[l2, below right=\dy mm and \dx mm of l12] (l23) {};

\node[l2, below right=\dy mm and \dx mm of l21] (l31) {};
\node[l2, below right=\dy mm and \dx mm of l22] (l32) {};

\node[empty, below right=\dy mm and 2mm of l31] (output) {};

\foreach \i in {1,2}{
    \foreach \j in {1,2,3}{
        \draw[shorten >=1pt] (l1\i) -- (l2\j);}}
 
\foreach \i in {1,2,3}{
    \foreach \j in {1,2}{
        \draw[shorten >=1pt] (l2\i) -- (l3\j);}}

\draw[arrow] (output.east) -> +(1,0) node[empty](arr2){};

\node[xshift=1cm, rounded corners=2mm, minimum size=2cm, path picture={
    \node at (path picture bounding box.center){
        \includegraphics[width=2cm]{imgs/pred.jpeg}};
}] (pred) at(arr2.east) {};
\node[above=14mm of pred] {$\hat{y}$};

\node[below=15mm of l23] (mask) {};

\draw[arrow] (gray.south east) -> (mask.north west);
\draw[arrow] (pred.south west) -> (mask.north east);

% MASKER
\node[empty] (input) at(mask.south) {};

\node[l1, below left=2mm and \dy mm of input] (l11) {};
\node[l1, below right=2mm and \dy mm of input] (l12) {};

\node[l1, below left=\dx mm and \dy mm of l11] (l21) {};
\node[l1, below right=\dx mm and \dy mm of l11] (l22) {};
\node[l1, below right=\dx mm and \dy mm of l12] (l23) {};
\node[rotate=270, right=5mm of l23]{\footnotesize Masking Model};

\node[l1, below right=\dx mm and \dy mm of l21] (l31) {};
\node[l1, below right=\dx mm and \dy mm of l22] (l32) {};

\node[empty, below right=2mm and \dy mm of l31] (output) {};

\foreach \i in {1,2}{
    \foreach \j in {1,2,3}{
        \draw[shorten >=1pt] (l1\i) -- (l2\j);}}
 
\foreach \i in {1,2,3}{
    \foreach \j in {1,2}{
        \draw[shorten >=1pt] (l2\i) -- (l3\j);}}

\draw[arrow] (output.south) -> +(0,-1) node[empty](arr3){};
\node[yshift=-1cm, rounded corners=2mm, minimum size=2cm, path picture={
    \node at (path picture bounding box.center){
        \includegraphics[width=2cm]{imgs/mask.png}};
}] (mask) at(arr3.south) {};
\node[below=14mm of mask] {$m$};

\begin{scope}[xshift=8cm, yshift=-3.5cm]
\node[rounded corners=2mm, minimum size=2cm, path picture={
    \node at (path picture bounding box.center){
        \includegraphics[width=2cm]{imgs/00000000.jpg}};
}] (y) at(0,0) {};
\node[above=14mm of y] {$y$};
\node[right=15mm of y] (odot) {\Large$\odot$};
\node[right=15mm of odot, rounded corners=2mm, minimum size=2cm, path picture={
    \node at (path picture bounding box.center){
        \includegraphics[width=2cm]{imgs/mask.png}};
}] (m) {};
\node[above=14mm of m] {$m$};
\node[right=15mm of m] (eq) {\Large$=$};
\node[right=15mm of eq, rounded corners=2mm, minimum size=2cm, path picture={
    \node at (path picture bounding box.center){
        \includegraphics[width=2cm]{imgs/y_m.png}};
}] (ym) {};
\node[above=14mm of ym] {$y \odot m$};
\end{scope}

\begin{scope}[xshift=8cm, yshift=-6cm]
\node[rounded corners=2mm, minimum size=2cm, path picture={
    \node at (path picture bounding box.center){
        \includegraphics[width=2cm]{imgs/pred.jpeg}};
}] (y_hat) at(0,0) {};
\node[below=14mm of y_hat] {$\hat{y}$};
\node[right=15mm of y_hat] (odot) {\Large$\odot$};
\node[right=15mm of odot, rounded corners=2mm, minimum size=2cm, path picture={
    \node at (path picture bounding box.center){
        \includegraphics[width=2cm]{imgs/mask.png}};
}] (m) {};
\node[below=14mm of m] {$m$};
\node[right=15mm of m] (eq) {\Large$=$};
\node[right=15mm of eq, rounded corners=2mm, minimum size=2cm, path picture={
    \node at (path picture bounding box.center){
        \includegraphics[width=2cm]{imgs/y_hat_m.png}};
}] (y_hatm) {};
\node[below=14mm of y_hatm] {$\hat{y} \odot m$};
\end{scope}



\end{tikzpicture}
\caption{\label{fig:model}High level view of our model: 1) $x$ is the input to the colorization model. 2) $x$ and $\hat{y}$, the colorized image, are the input to the masking model which predicts the uncertainty mask $m$. 3) $y$ is the reference image and with high probability the distortion between the masked images, $y \odot m$ and $\hat{y} \odot m$ is low.}
\end{figure}

\begin{algorithm}
\caption{\label{alg:calibration}Finding $\lambda_i$}
\centering
\begin{minted}{python}
def find_lambda(*, mask, y, y_hat, d, alpha, eps=1e-3):
    l, h = eps, 1 / eps
    lambda = (h + l) / 2
    while h - l > eps:
        lambda = (h + l) / 2
        loss = d(
            y * (lambda * mask).clamp(0, 1), 
            y_hat * (lambda * mask).clamp(0, 1))
            
        if loss > alpha:
            h = m
        else:
            l = m

    return lambda
\end{minted}
\end{algorithm}


\section{Experiments}
\todo{Compare with quantile regression?}
First, we train models for the relevant tasks.
We experiment with two data sets: 1) a subset of 1,803,460/36,500 256x256 images from the Places365 data set~\cite{places365} for training/validation respectively, and 2) 1,539,618/47.582 256x256 patches from the TEMCA2 data set~\cite{temca2} for training/validation respectively.
TEMCA2 is a huge data set with 7,062 8192x8192 uncompressed images with a total size of ~26TB of data.
As some of the images contain large amount of black background, we decided to take patches only from images larger than 36MB.
A manual examination of a random sample of those images verified that they do not contain such a background.
We randomly split the patches into train and validation sets.
We use these data sets for the following tasks:

\paragraph{Image Colorization}
For this task we use the places365 data set. 
We convert the images to gray-scale and the goal is to reconstruct the original colors of the image.
\paragraph{Image Completion}
We use gray-scale images from the places365 data set from which we remove a vertical and horizontal stripes of 32 pixel width. 
The model's objective is to reconstruct the missing pixels.
\paragraph{Super Resolution}
We use the 256x256 patchs from the TEMCA2 data set and downscale them to 32x32 images. 
The goal of the model is to reconstruct the original patch.

Figure~\ref{fig:tasks} shows a sample input and output for each one of the above tasks.

\begin{figure}
    \centering
    \begin{tabular}{c c c}
        \includegraphics[width=.25\textwidth]{imgs/color.jpg}
        & \includegraphics[width=.25\textwidth]{imgs/completion.jpg}
        & \includegraphics[width=.25\textwidth]{imgs/sr.png}
        \\
        \includegraphics[width=.25\textwidth]{imgs/00000000.jpg}
        & \includegraphics[width=.25\textwidth]{imgs/color.jpg}
        & \includegraphics[width=.25\textwidth]{imgs/00000000.png}
    \end{tabular}

    \caption{\label{fig:tasks}
    The three tasks we experimented with: 1) Image Colorization on the left column 2) Gray-scale Image Completion on the middle column, and 3) Super Resolution on the right column.}
\end{figure}

\subsection{Experimental Details}
We use the same model architecture for all tasks, that is a 8 layer U-Net\footnote{This is the same architecture as our masking model as well. This choice was done for simplicity and compatibility with previous work.}.
For each task we train both a simple regressor and a conditional generator (G) with an adversarial discriminator (D) which we refer to as conditional GAN or simply GAN. 
As in~\cite{pix2pix} the generator observes the input but it does not have an access to a random noise.
Our discriminator is a 4 layer convolution network with a fully connected head.
We use the L1 loss as the objective for the regressor and for the conditional GAN we use the same objective as in~\cite{pix2pix}, that is:
\begin{equation}
    \arg \min_G \max_D \mathcal{L}_{\text{cGAN}}(G, D) + \lambda\mathcal{L}_\text{L1}(G)
\end{equation}
where we set $\lambda = 20$ and
\begin{equation}
    \mathcal{L}_{\text{cGAN}}(G, D) = \mathbb{E}_{x,y}[\log D(x, y)] + \mathbb{E}[\log(1 - d(x, G(x, y)))]
\end{equation}

All models are trained for two epochs using the Adam optimizer with a learning rate equal to $1\text{e-}5$ and a batch size equel to 50. 
We report the average L1, LPIPS~\cite{lpips} and DISTS~\cite{dists} in Table~\ref{tab:l1} as well as the standard deviation.
We also report the correlation between L1 and the other two metrics for the colorization task in Table~\ref{tab:l1corr}.

\begin{table}
\centering
\begin{tabular}{lcccccc}

\toprule
& \multicolumn{2}{c}{Colorization} 
& \multicolumn{2}{c}{Image Completion}  
& \multicolumn{2}{c}{Super Resolution} 
\\      
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
\cmidrule(lr){6-7}
& Regressor & GAN                
& Regressor & GAN                       
& Regressor & GAN
\\\midrule
L1 & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$
\\
LPIPS & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$
\\
DISTS & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$

\\\bottomrule
\end{tabular}

\caption{
\label{tab:l1}
\todo{}}
\end{table}

\begin{table}
\centering
\begin{tabular}{lcccc}

\toprule
& \multicolumn{2}{c}{LPIPS} 
& \multicolumn{2}{c}{DISTS}  
\\      
\cmidrule(lr){2-3}
\cmidrule(lr){4-5}
& Regressor & GAN                
& Regressor & GAN                       
\\\midrule
L1 & $99\pm99$ & $99\pm99$ & $99\pm99$ & $99\pm99$

\\\bottomrule
\end{tabular}

\caption{\label{tab:l1corr}
\todo{Caption}}
\end{table}

For the masking model we use a 8 layers U-Net architecture as well.
The masking model is trained using the prediction of the other models with a target loss function.
There are 18 possible combinations of \textbf{Task} $\times$ \textbf{Model} $\times$ \textbf{Loss}, out of which we chose to train a masking model and evaluate it on the following combinations:
\begin{enumerate}
    \label{list:comb}
    \item Colorization, Regression, L1
    \item Colorization, GAN, LPIPS
    \item Image Completion, GAN, L1
    \item Image Completion, GAN, DISTS
    \item Super Resolution, Regression, L1
    \item Super Resolution, GAN, L1
\end{enumerate}

\subsection{Evaluation}
First we report the performance of our models on the validation sets for the three tasks.
Table~\ref{tab:model-eval} shows the mean absolute error (MAE) as well as the FID score~\cite{fid} where applicable.
Note that training a well performing model for these tasks is not in the scope of this paper and we are satisfied with the reported results.

\begin{table}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{rccc}
        \toprule
        && MAE   & FID 
        \\ \midrule
        \multirow{2}*{Colorization} & Regression & $99\pm 99$  & $99\pm 99$
        \\ & GAN & $99\pm 99$ & $99\pm 99$
        \\ \midrule
        \multirow{2}*{Image Completion} & Regression & $99\pm 99$  & $99\pm 99$
        \\ & GAN & $99\pm 99$ & $99\pm 99$
        \\ \midrule
        \multirow{2}*{Super Resolution} & Regression & $99\pm 99$  & $99\pm 99$
        \\ & GAN & $99\pm 99$ & $99\pm 99$
        \\ \bottomrule
    \end{tabular}
    \caption{\label{tab:model-eval}Caption}
\end{table}

% For evaluation we split the validation test into calibration and test sets.
% The sizes of the calibration and test sets are 999/999 and 999/999 for the places365 and TEMCA2 data-sets respectively.

To evaluate our masking model and calibration procedure first we need to make sure that the heuristic notion of mask is reasonable.
To verify this we check that the mean absolute error between $m$ and $\hat{m}$ is low and that the size of $\hat{m}$ is highly correlated with the size of $m$ as well as with the distortion it tries to minimize, i.e. one of L1, LPIPS, DISTS.
Table~\ref{tab:mask-eval1} summarize these results. 
\todo{Metrics Insights}

\begin{table}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{rcccc}
        \toprule
        &&& MAE   & CORR 
        \\ \midrule
        \multirow{2}*{Colorization} & Regression & L1 & $99\pm 99$  & $99\pm 99$
        \\ & GAN & LPIPS  & $99\pm 99$ & $99\pm 99$
        \\ \midrule
        \multirow{2}*{Image Completion} & \multirow{2}*{GAN} & L1  & $99\pm 99$ & $99\pm 99$
        \\ && DISTS  & $99\pm 99$ & $99\pm 99$
        \\ \midrule
        \multirow{2}*{Super Resolution} & Regression & L1  & $99\pm 99$ & $99\pm 99$
        \\ & GAN & L1  & $99\pm 99$ & $99\pm 99$
        \\ \bottomrule
    \end{tabular}
    \caption{\label{tab:mask-eval1}Caption}
\end{table}

Now we evaluate our solution end to end.
We set $\beta = 0.9$ (see Equation~\ref{eq:goal}) and set $\alpha$ to the minimum distortion obtained among the validation set for each of the individual combinations listed in~\ref{list:comb}. 
We start by evaluating the size of the calibrated masks as, under the same guarantees, smaller masks are preferred.
We establish two baselines to compare with, in the first one (UNI) we compute the maximal scalar, $\mu \in [0, 1]$, such that at least $90\%$ of our calibration set satisfies $d(y \cdot \mu, \hat{y} \cdot \mu) \leq \alpha$.
Note that this is the same as using our calibration procedure on a heuristic that always produce the $\hat{m} = \vv{1}$.
In the second baseline (OPT) we compute a mask by applying gradient decent using the gradient of $d_m$.
We use a learning rate of $999$ and repeat until the first time the distortion between the masked images dropped below the desired threshold.
In a sense, this is the optimal solution.
Table~\ref{tab:mask-size} compare the average mask size for each of the evaluated combinations.

\begin{table}
    \renewcommand{\arraystretch}{1.3}
    \centering
    \begin{tabular}{rccccc}
        \toprule
        &&& Our   & UNI & GRAD
        \\ \midrule
        \multirow{2}*{Colorization} & Regression & L1 & $99\pm 99$  & $99\pm 99$ & $99\pm 99$
        \\ & GAN & LPIPS  & $99\pm 99$ & $99\pm 99$ & $99\pm 99$
        \\ \midrule
        \multirow{2}*{Image Completion} & \multirow{2}*{GAN} & L1  & $99\pm 99$ & $99\pm 99$ & $99\pm 99$
        \\ && DISTS  & $99\pm 99$ & $99\pm 99$ & $99\pm 99$
        \\ \midrule
        \multirow{2}*{Super Resolution} & Regression & L1  & $99\pm 99$ & $99\pm 99$ & $99\pm 99$
        \\ & GAN & L1  & $99\pm 99$ & $99\pm 99$ & $99\pm 99$
        \\ \bottomrule
    \end{tabular}
    \caption{\label{tab:mask-size}Caption}
\end{table}

We also compute the correlation between the size of the masks obtained by our method and OPT as higher correlation indicates better adaptivity, see Section~3.1 in~\cite{gentle}.
\todo{Summarize correlation}


\section{Conclusion}
\todo{Finish conclusion}

\bibliography{main} 
\bibliographystyle{ieeetr}
\end{document}






==> text/comments.tex <==
\begin{enumerate}
    \color{blue}
    \item Our calibrated mask is inverse proportional to the predicted "mask". It would be clearer if we say that we try to predict the expected distortion and then use it to obtain a mask.
    \item Compute confidence intervals for the evaluation (mask size and correlation).
    \item Maybe we should generate a synthetic dataset, e.g. synthetic colorization where each image contains several rectangles and their color distribution related to their size and shape?
    \item Assume we would like to predict the expected distortion, how do we generalize this to structural distortion measures? i.e. what should we predict for each pixel?
\end{enumerate}
